Monge-Kantorovich Fitting With Sobolev Budgets

Given $m < n$, we consider the problem of ``best'' approximating an $n\text{-d}$ probability measure $\rho$ via an $m\text{-d}$ measure $\nu$ such that $\mathrm{supp}\ \nu$ has bounded total ``complexity.'' When $\rho$ is concentrated near an $m\text{-d}$ set we may interpret this as a manifold learning problem with noisy data. However, we do not restrict our analysis to this case, as the more general formulation has broader applications. We quantify $\nu$'s performance in approximating $\rho$ via the Monge-Kantorovich (also called Wasserstein) $p$-cost $\mathbb{W}_p^p(\rho, \nu)$, and constrain the complexity by requiring $\mathrm{supp}\ \nu$ to be coverable by an $f : \mathbb{R}^{m} \to \mathbb{R}^{n}$ whose $W^{k,q}$ Sobolev norm is bounded by $\ell \geq 0$. This allows us to reformulate the problem as minimizing a functional $\mathscr J_p(f)$ under the Sobolev ``budget'' $\ell$. This problem is closely related to (but distinct from) principal curves with length constraints when $m=1, k = 1$ and an unsupervised analogue of smoothing splines when $k > 1$. New challenges arise from the higher-order differentiability condition. We study the ``gradient'' of $\mathscr J_p$, which is given by a certain vector field that we call the barycenter field, and use it to prove a nontrivial (almost) strict monotonicity result. We also provide a natural discretization scheme and establish its consistency. We use this scheme as a toy model for a generative learning task, and by analogy, propose novel interpretations for the role regularization plays in improving training.

==> preamble.tex <==
% For `\shortintertext{}` and other things.
\usepackage{mathtools}
%
\usepackage{amsmath, amssymb}
\makeatletter

% --------------------------- Delimiters --------------------------- %
%% See https://tex.stackexchange.com/a/1744
% auto-sized stuff
\let\size@autol\left  \let\size@autor\right \let\size@autom\middle

% Stop expansion if we have the base thing
\let\size@basel\relax \let\size@baser\relax \let\size@basem\relax

% Sizes
\let\size@bigl\bigl   \let\size@bigr\bigr   \let\size@bigm\big
\let\size@Bigl\Bigl   \let\size@Bigr\Bigr   \let\size@Bigm\Big
\let\size@biggl\biggl \let\size@biggr\biggr \let\size@biggm\bigg
\let\size@Biggl\Biggl \let\size@Biggr\Biggr \let\size@Biggm\Bigg

\newcommand{\ldelim}{\relax}
\newcommand{\rdelim}{\relax}
\newcommand{\mdelim}{\relax}

\newcommand{\size@command}[4]{{%
  \def\ldelim{\csname size@#1l\endcsname}% tack on size to l delim
  \def\rdelim{\csname size@#1r\endcsname}% tack on size to r delim
  \def\mdelim{\csname size@#1m\endcsname}%
  \ldelim#2#4\rdelim#3% put the stuff in between
}}

% Define new delimiter commands with ease!
% #1 name #2 ldelim #3 rdelim
\newcommand{\newdelimcommand}[3]{%
  \expandafter\newcommand\csname size@#1@st\endcsname[1]{%
    \size@command{base}{#2}{#3}{##1}}% ##1 content
  \expandafter\newcommand\csname size@#1@ns\endcsname[2][auto]{%
    % ##1 size ##2 content
    \size@command{##1}{#2}{#3}{##2}}%
  \expandafter\DeclareRobustCommand\csname#1\endcsname{%
    \@ifstar{\csname size@#1@st\endcsname}{\csname size@#1@ns\endcsname}%
  }%
}

\makeatother

% syntactically named delimiters
\newdelimcommand{braces}{\lbrace}{\rbrace}
\newdelimcommand{angles}{\langle}{\rangle}
\newdelimcommand{verts}{\lvert}{\rvert}
\newdelimcommand{Verts}{\lVert}{\rVert}
\newdelimcommand{brackets}{[}{]}
\newdelimcommand{parens}{(}{)}
\newdelimcommand{bras}{\langle}{\rvert}
\newdelimcommand{kets}{\lvert}{\rangle}
\newdelimcommand{floors}{\lfloor}{\rfloor}
\newdelimcommand{ceils}{\lceil}{\rceil}

% Half-open
\newdelimcommand{pnbks}{(}{]}
\newdelimcommand{bkpns}{[}{)}

% semantically named delimiters
\newcommand{\set}{\braces}
\newcommand{\abs}{\verts}
\newcommand{\norm}{\Verts}
\newcommand{\pn}{\parens}
\newcommand{\ip}{\angles}
\newcommand{\bk}{\brackets}
\newcommand{\bra}{\bras}
\newcommand{\ket}{\kets}
\newcommand{\floor}{\floors}
\newcommand{\ceil}{\ceils}
\newcommand{\pb}{\pnbks}
\newcommand{\bp}{\bkpns}

% Automagic `such that' for set comprehension. Inside an automagic
% delimiter command, the vertical bar will resize appropriately
% Example:
%   \set{ x \in W \MID x > 0 }
\newcommand{\MID}{\mspace{5mu}\mdelim\vert\mspace{5mu}}



\usepackage{booktabs}
\usepackage{changepage}

\usepackage{multicol}

\usepackage{float, subcaption}


\usepackage[breakable, skins]{tcolorbox}


\usetikzlibrary{calc}

\numberwithin{equation}{section}

\allowdisplaybreaks


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Theorem environments, etc.
\usepackage{amsthm}

\let\oldqed\qed
\renewcommand{\qed}{\hfill $\blacksquare$}

\theoremstyle{plain}% default
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}

% This is for getting numbering right when we repeat a theorem in the
% intro vs. later
\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
  \def\rep@title{#2 \ref{##1}}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}}
\makeatother
\newreptheorem{theorem}{Theorem}


\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{problem}{Problem}
\newtheorem{question}{Question}
\newtheorem{example}[theorem]{Example}
\newtheorem{counterexample}[theorem]{Counterexample}
\newtheorem{remark}[theorem]{Remark}


% Same but for definitions
\makeatletter
\newtheorem*{rep@definition}{\rep@title}
\newcommand{\newrepdefinition}[2]{%
\newenvironment{rep#1}[1]{%
  \def\rep@title{#2 \ref{##1}}%
 \begin{rep@definition}}%
 {\end{rep@definition}}}
\makeatother
\newrepdefinition{definition}{Definition}

\usepackage{hyperref}
\hypersetup{colorlinks={true},linkcolor={blue},citecolor=green}
\usepackage[capitalize]{cleveref}

\AddToHook{cmd/appendix/before}{\crefalias{section}{appendix}}
\AddToHook{cmd/appendix/before}{\crefalias{subsection}{appendix}}

\AddToHook{env/theorem/begin}{\crefalias{theorem}{theorem}}
\AddToHook{env/lemma/begin}{\crefalias{theorem}{lemma}}
\AddToHook{env/corollary/begin}{\crefalias{theorem}{corollary}}
\AddToHook{env/proposition/begin}{\crefalias{theorem}{proposition}}

\AddToHook{env/problem/begin}{\crefalias{definition}{problem}}
\AddToHook{env/example/begin}{\crefalias{definition}{example}}
\AddToHook{env/remark/begin}{\crefalias{definition}{remark}}
\AddToHook{env/question/begin}{\crefalias{definition}{question}}
\AddToHook{env/counterexample/begin}{\crefalias{definition}{counterexample}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% General math macros

% For bold math things
\usepackage{bm}

% For leftbar environment (useful in proving lemmas, etc)
\usepackage[framemethod=tikz]{mdframed}

% Enumeration
\usepackage{enumitem}

% Use a different script font
\usepackage[scr=esstix]{mathalfa}

% ----------------------- General Math Stuff ----------------------- %

% Useful shortcuts for when typing is just too hard
\newcommand*{\mrm}[1]{{\mathrm{#1}}}
\newcommand*{\mbb}[1]{{\mathbb{#1}}}
\newcommand*{\mc}[1]{{\mathcal{#1}}}
\newcommand*{\mb}[1]{{\mathbf{#1}}}
\newcommand*{\ms}[1]{{\mathscr{#1}}}
\newcommand*{\msf}[1]{{\mathsf{#1}}}

% Avoid exiting math mode for such that
\newcommand{\st}{\mrm{\ s.t.\ }}

% common fields
\newcommand{\CC}{\mathbb{C}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\NN}{\mathbb{N}}

% Widetilde shortcut. Need the prepended `{}' because of this issue
% here: https://tex.stackexchange.com/q/470175
\newcommand{\wt}[1]{{}\widetilde{#1}}

% Overline, more tersely. For things like closures, etc.
\newcommand{\ol}[1]{\overline{#1}}


% Total differential
\newcommand{\dd}{\mathop{}\mspace{1mu} d}

% Injection notation
\newcommand{\into}{\hookrightarrow}

% Optimizations
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

% For properly aligning things w/ neg numbers in matrix environments
\newcommand{\ph}{\phantom{-}}

% Uniform convergence
\newcommand{\uconv}{\xrightarrow{u}}

% Weak convergence
\newcommand{\wconv}{\rightharpoonup}

% Sequences that increase to a value
\newcommand{\incto}{\nearrow}
\newcommand{\decto}{\searrow}

% Support
\DeclareMathOperator{\supp}{supp}

% Essential supremum / infimum
\DeclareMathOperator*{\esssup}{ess\,sup}
\DeclareMathOperator*{\essinf}{ess\,inf}

% Identity
\newcommand{\id}[1][]{\operatorname{id}_{#1}}

% Add sign operator
\DeclareMathOperator{\sgn}{sgn}

% Direct sums
\newcommand{\osum}{\bigoplus}

% ----------------------- Probabilistic stuff ---------------------- %

% Expected value
\newcommand{\EE}{\mathbb{E}}

% Variance
\newcommand{\Var}{\operatorname{Var}}

% For typesetting algorithms
\RequirePackage[ruled, vlined, linesnumbered]{algorithm2e}



% leftbar
\newmdenv[
  skipabove=5,
  skipbelow=5,
  innerleftmargin = .5em,
  innertopmargin = .5em,
  innerbottommargin = .5em,
  innerrightmargin = 0pt,
  rightmargin = 0pt,
  leftmargin = 2em,
  linewidth = 2pt,
  topline = false,
  rightline = false,
  bottomline = false
  ]{leftbar}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{xspace}
\usepackage{xcolor,calc}
\usepackage{tikzpagenodes,linegoal}
\usetikzlibrary{calc}
\usepackage{tcolorbox}

% ------------------------------------------------------------------ %


\newcommand{\ie}{i.e.\xspace{}}
\newcommand{\eg}{e.g.\xspace{}}
\newcommand{\cf}{c.f.\xspace{}}

% ------------------------------------------------------------------ %

\newcommand{\reffnc}{\hyperref[eq:fnc-def]{\ensuremath \fnc}}
\newcommand{\refbudgmin}{\hyperref[eq:budgmin-def]{\ensuremath \budgmin}}
\newcommand{\reffmin}{\hyperref[eq:fmin-def]{\ensuremath \fmin}}
\newcommand{\refbnc}{\hyperref[eq:bnc-def]{\ensuremath \bnc}}
\newcommand{\refambf}{\hyperref[eq:ambf-def]{\ensuremath \ambf}}
\newcommand{\refpfdset}{\hyperref[eq:pfdset-def]{\ensuremath \pfdset}}
\newcommand{\refpfiset}{\hyperref[eq:pfiset-def]{\ensuremath \pfiset}}
\newcommand{\refpl}{\hyperref[term:PL]{PL} \xspace{}}


%%% General macros
%
% Diameter of a set
\DeclareMathOperator{\diam}{diam}
%
% serif lettering
\newcommand{\sfn}{\mathsf{N}}
\newcommand{\sfnj}{{\sfn_{\msf j}}}
%
% Almost sure equality
\newcommand{\eqas}{\ensuremath \overset{\rm a.s.}{=}}
%
% Set of all probability measures on a set
\newcommand{\pmeas}{\ensuremath \mc P}
%
% Generic set element
\newcommand{\tinybox}{\,\scalebox{.6}{\ensuremath \square}\,}
%
% Domain
\newcommand{\ddim}{\ensuremath m} % domain dimension
\newcommand{\rddim}{\ensuremath \RR^\ddim}
\newcommand{\dset}{\ensuremath X} % domain set
\newcommand{\dpt}{\ensuremath x}  % point in the domain
\newcommand{\dptspec}{\dpt_{\specind}}
\newcommand{\dmeas}{\ensuremath\mu} % domain set measure
\newcommand{\dsn}{\mathsf{\dset_N}} % empirical measure on dset
\newcommand{\dsub}{\dset^\circ}
\newcommand{\dptsfi}{\ensuremath \msf{\dpt}_{\msf i}}
\newcommand{\dptsfj}{\ensuremath \msf{\dpt}_{\msf j}}
%
% Codomain
\newcommand{\cdim}{\ensuremath n}
\newcommand{\rcdim}{\ensuremath \RR^\cdim}
\newcommand{\cset}{\ensuremath \Omega} % codomain set
\newcommand{\csetepssfj}{\ensuremath \cset_{\epssfj}}
\newcommand{\cpt}{\ensuremath \omega} % point in the codomain
\newcommand{\cmeas}{\ensuremath \rho} % codomain set measure
\newcommand{\cunif}{\cmeas_{\rm unif}}
%
% Image set
\newcommand{\iset}{\ensuremath Y} % image set
\newcommand{\isn}{\mathsf{\iset_N}}
\newcommand{\isneps}{\mathsf{\iset}_{\sfn, \varepsilon}}
\newcommand{\isnepsj}{\mathsf{\iset}_{\sfn, \epssfj}}
\newcommand{\isnout}{\mathsf{\iset}_{\sfn, \mathrm{out}}}
\newcommand{\isnj}{\mathsf{\iset}_{\sfnj}}
\newcommand{\ipt}{\ensuremath y}  % point in the image
\newcommand{\iptsf}{\ensuremath \mathsf{\ipt}}
\newcommand{\iptsfi}{\ensuremath \iptsf_{\mathsf{i}}}
\newcommand{\iptsfj}{\ensuremath \iptsf_{\mathsf{j}}}
\newcommand{\iptsfn}{\ensuremath \iptsf_{\sfn}}
\newcommand{\imeas}{\ensuremath\nu} % image set measure
%
% Injectivity set
\newcommand{\ninjdset}{\wt \dset}
\newcommand{\ninjiset}{\wt \iset}
%
% Unequal dim OT macros
\newcommand{\uneqdd}{\ensuremath \ddim}
\newcommand{\uneqds}{\ensuremath \dset}
\newcommand{\uneqdp}{\ensuremath \dpt}
\newcommand{\uneqdm}{\ensuremath \dmeas}
\newcommand{\uneqid}{\ensuremath \cdim}
\newcommand{\uneqis}{\ensuremath Y}
\newcommand{\uneqip}{\ensuremath y}
\newcommand{\uneqim}{\ensuremath \nu}
\newcommand{\uneqf}{\ensuremath \fmap}
\newcommand{\uneqtp}{\ensuremath \gamma}
\newcommand{\uneqtps}{\ensuremath \Gamma}
\newcommand{\besttp}{\ensuremath \uneqtp^*}
\newcommand{\bestertp}{\ensuremath \wt \uneqtp^*}
%
% Zero subscript
\newcommand{\dz}{\dpt_0}
%
% Epsilon version of things
\newcommand{\iseps}{\iset_\varepsilon}
\newcommand{\epssfj}{\ensuremath \varepsilon}
\newcommand{\epssfn}{\varepsilon_{\sfn}}
\newcommand{\dsfi}{\delta_{\msf i}}
\newcommand{\dsfj}{\delta_{\msf j}}
%
% The map \fillmap : X \to Y giving our filling
\newcommand{\fmap}{\ensuremath f}
\newcommand{\fhat}{\widehat \fmap}
\newcommand{\ftilde}{\wt \fmap}
\newcommand{\feps}{\fmap_{\varepsilon}}
\newcommand{\finv}{\fmap^{-1}}
\newcommand{\fbudg}{\fmap_\budg}
\newcommand{\fbt}{\ftilde_\budg}
\newcommand{\fn}{\fmap_N}
\newcommand{\fmin}{\cpt_{{\cost}}}
\newcommand{\fnc}{\cpt_{{\objf}}}
\newcommand{\finf}{\fmap_\infty}
\newcommand{\fj}{\fmap_j}
\newcommand{\fjp}{\fmap_j^+}
\newcommand{\fjm}{\fmap_j^-}
\newcommand{\fjseq}{\set{\fj}_{j=1}^\infty}
\newcommand{\fcompj}{\fmap^j}
\newcommand{\fz}{\fmap_0}
\newcommand{\fgood}{\fmap_{\rm good}}
\newcommand{\fbad}{\fmap_{\rm bad}}
\newcommand{\gmap}{\ensuremath g}
\newcommand{\fepssf}{\msf{\fmap}_{\varepsilon_{\sfn}}}
\newcommand{\fthet}{\fmap^\theta}
\newcommand{\fthetn}{\fthet_N}
%
% Sobolev things
\newcommand{\sobw}{\ensuremath W}
\newcommand{\sobk}{\ensuremath k} % order of weak derivatives
\newcommand{\sobp}{\ensuremath q}
\newcommand{\wkp}{\sobw^{\sobk, \sobp}}
\newcommand{\wkpsets}{\sobw^{\sobk, \sobp}(\dset; \cset)}
%
% U
\newcommand{\wkpu}{\sobw^{\sobk, \sobp}(\dsub)}
\newcommand{\wkpuo}{\sobw^{\sobk, \sobp}(\dsub; \cset)}
\newcommand{\wkpur}{\sobw^{\sobk, \sobp}(\dsub; \rcdim)}
\newcommand{\sobnorm}[1]{\norm{#1}_{\wkpsets}}
\newcommand{\mind}{\ensuremath \alpha} % multiindex
%
% C^k things
\newcommand{\holda}{\ensuremath a}
\newcommand{\holdr}{\ensuremath \gamma}
\newcommand{\holdur}{C^{\holda, \holdr}(\ol \dsub; \rcdim)}
\newcommand{\holdxc}{C^{\holda, \holdr}(\dset; \cset)}
%
% Closest point projection
\newcommand{\pmap}{\ensuremath \pi}
\newcommand{\pmapset}{\ensuremath \pi}
\newcommand{\psin}{\hat \pmap_{\isn}}
\newcommand{\psinj}{\hat \pmap_{\msf{N_j}}}
\newcommand{\psineps}{\hat \pmap_{\isn, \varepsilon}}
\newcommand{\pf}{\pmap_{\fmap}}
%
% Closest point projection onto $\iset$
\newcommand{\pfi}{\hat \pmap_\iset}
\newcommand{\pfim}{\pfi^*}
\newcommand{\pfis}{\pmapset_\iset}
\newcommand{\pfiset}{\ensuremath \hat \Pi_\iset}
\newcommand{\pfiinv}{\pfi^{-1}}
\newcommand{\pfiminv}{(\pfim)^{-1}}
%
% Closest point projection into $\dset$
\newcommand{\pfd}{\ensuremath \hat \pmap_\dset}
\newcommand{\pfdm}{\pfd^*}
\newcommand{\pfds}{\pmapset_\dset}
\newcommand{\pfdset}{\hat \Pi_\dset}
\newcommand{\pfdepsm}{\hat \pmap^*_{\varepsilon, \dset}}
\newcommand{\pfdepss}{\pmapset_{\varepsilon, \dset}}
\newcommand{\pfdinv}{\pfd^{-1}}
\newcommand{\pfdminv}{(\pfdm)^{-1}}

%%% Measurable selection stuff
\newcommand{\optset}{\ensuremath Z}
\newcommand{\optpt}{\ensuremath z}
%
% Projection onto $\cset$
\newcommand{\projc}{\ensuremath \mrm{proj}_\cset}
%
% The closed set used in the theorem thing
% seldom == selection domain
\newcommand{\seldom}{\ensuremath D}
\newcommand{\seldomc}{\seldom_\cpt}
\newcommand{\seldomeps}{\seldom^\varepsilon}

% lower-semicontinuous function used in the measurable selection
% theorem
\newcommand{\lscf}{\ensuremath h}
\newcommand{\lscft}{\wt \lscf}
\newcommand{\lscfeps}{\lscf_\varepsilon}
\newcommand{\lscfm}{\lscf^*} % m for min
\newcommand{\lscftm}{\lscft^*} % m for min
\newcommand{\lscfepsm}{\lscfeps^*}
%
% graph
\newcommand{\graph}{\ensuremath \mrm{graph}}
%
% Need to frequently refer to a vector in the codomain
\newcommand{\cdv}{\ensuremath v}
\newcommand{\cdvz}{\cdv_0}
\newcommand{\cdvh}{\hat \cdv}
%
% Some common pushforwards
\newcommand{\cpushi}{\ensuremath \imeas_\cmeas}
\newcommand{\cpushih}{\imeas_{\pfi}}
\newcommand{\cpushihm}{\imeas_{\pfim}}
\newcommand{\cpushdh}{\dmeas_{\pfd}}
\newcommand{\cpushdhm}{\dmeas_{\pfdm}}
\newcommand{\cpush}{\ensuremath \imeas_\cmeas}
\newcommand{\cpushsf}{\ensuremath \imeas_{\psin}}
%
% Disintegration
\newcommand{\cmdpt}{\cmeas_\dpt}
\newcommand{\cmipt}{\cmeas_\ipt}
\newcommand{\cmiptsf}{\cmeas_{\mathsf{\ipt}}}
\newcommand{\cmiptsfn}{\cmeas_{\iptsf, \psin}}
\newcommand{\cmipth}{\cmeas_{\ipt, \pfi}}
\newcommand{\cmipthm}{\cmeas_{\ipt, \pfim}}
\newcommand{\cmdpth}{\cmeas_{\dpt, \pfd}}
\newcommand{\cmdpthm}{\cmeas_{\dpt, \pfdm}}
%
% Barycenter field
\newcommand{\fbsymb}{\ensuremath F}
\newcommand{\fbs}{\fbsymb}
\newcommand{\fbd}{\fbsymb_\dset}
\newcommand{\fbdh}{\fbsymb_{\pfd}}
\newcommand{\fbdhm}{\fbsymb_{\pfdm}}
\newcommand{\fbi}{\fbsymb_\iset}
\newcommand{\fbih}{\fbsymb_{\pfi}}
\newcommand{\fbihm}{\fbsymb_{\pfim}}

\newcommand{\fbary}{\fbsymb_p}
\newcommand{\fbarysf}{\mathsf{\fbsymb}_{\psin}}
\newcommand{\fbarysfj}{\mathsf{\fbsymb}_{\psinj}}
\newcommand{\fbarys}{\ensuremath \mf F_\objp}



%%% Important objects
%
% Bump function
\newcommand{\bump}{\ensuremath \eta}
\newcommand{\smoothstep}{\sigma}
\newcommand{\smoothdip}{\wt \sigma}

% Mollifier
\newcommand{\moll}{\ensuremath \varphi}
\newcommand{\mthet}{\ensuremath \moll_\theta}

%
% Perturbation
\newcommand{\pert}{\ensuremath \xi}
\newcommand{\perty}{\pert_\iset}
\newcommand{\perteps}{\pert_\varepsilon}

% Making sf math symbols non-slanted
\newsavebox{\foobox}
\newcommand{\slantbox}[2][0]{\mbox{%
        \sbox{\foobox}{#2}%
        \hskip\wd\foobox
        \pdfsave
        \pdfsetmatrix{1 0 #1 1}%
        \llap{\usebox{\foobox}}%
        \pdfrestore
}}
\newcommand\unslant[2][-.18]{\slantbox[#1]{$#2$}}

\DeclareSymbolFont{sfletters}{OML}{cmbrm}{m}{it}
\DeclareMathSymbol{\sxi}{\mathord}{sfletters}{"18}
\newcommand{\pertsf}{\ensuremath \unslant\sxi}
\newcommand{\pertsfn}{\ensuremath {\pertsf}_\sfn}

%
% The dimension we use in all of the radon measure proof things
\newcommand{\sld}{\ensuremath d}
\newcommand{\rsld}{\RR^\sld}
%
% The set of points that shrink nicely w.r.t Lebesgue
\newcommand{\slpts}{\ensuremath P}
\newcommand{\slptsj}{\ensuremath P_j}
\newcommand{\slptseps}{\slpts_\varepsilon}
%
% The x-specific growth factor thing
\newcommand{\constx}{\ensuremath c_\dpt}
%
% For the radon measure lemma
\newcommand{\sballs}{\ensuremath \mc B}
\newcommand{\sballseps}{\sballs_{\varepsilon}}
%
% Perturbation amplitude
\newcommand{\pertamp}{\ensuremath a}
%
% For the thing that's sort of like being a doubling measure but not
\newcommand{\dbfac}{\ensuremath \lambda}
\newcommand{\dbfacr}{\ensuremath \dbfac \smallr}
%
% Radius from the density theorem
\newcommand{\densr}{\ensuremath \delta}
\newcommand{\smallr}{\ensuremath r}
%
% `\bigr' and `\larger' are already taken
\newcommand{\bdensr}{\ensuremath B_{\densr}}
%
% The countable density stuff
\newcommand{\dsspec}{\dset_{\specind}}
\newcommand{\pertdens}{\pert_\densr}
%
% The special things we get from the density argument
\newcommand{\ind}{\ensuremath j}
\newcommand{\specind}{\ensuremath \ind_0}
%
% Special vector
\newcommand{\vspec}{\ensuremath v_{\specind}}
\newcommand{\fddset}{\ensuremath V} % Fiber direction dense set
\newcommand{\fibdir}{\ensuremath v}
\newcommand{\fibconst}{\ensuremath c}
%
% The two sets we break the integral up into. `id<...>' == `integral
% domain <...>'
\newcommand{\idz}{\ensuremath {A_0}}
\newcommand{\ido}{\ensuremath {A_1}}
\newcommand{\constz}{\ensuremath \beta_0}
\newcommand{\constzt}{\constz'}
\newcommand{\consto}{\ensuremath \beta_1}
%
% The integrand in the gradient proof
\newcommand{\gfunc}{\ensuremath g}
\newcommand{\geps}{\gfunc^\varepsilon}
%
% Medial axis
\newcommand{\ambset}{\ensuremath \mc A}
\newcommand{\ambf}{\ambset_{\fmap}}
\newcommand{\medax}{\ensuremath M}
\newcommand{\medset}{\ensuremath E}
\newcommand{\medpt}{\ensuremath v}
%
% Half spaces
\newcommand{\vjhat}{\ensuremath \hat v_j}
\newcommand{\halfpt}{\ensuremath \ipt_{\rm avg}}
\newcommand{\halfptj}{\ensuremath \ipt_j^{\rm avg}}
\newcommand{\halfspace}{\ensuremath H_{\ipt_0, \ipt_1}}
\newcommand{\halfspacej}{\ensuremath H_{\ipt_0, \ipt_j}}
%
% Polar cone
\DeclareMathOperator*{\pcone}{PCone}
\newcommand{\pcpt}{\ensuremath b}
\newcommand{\pcset}{\ensuremath B}
%
% Tangent cone stuff
\newcommand{\tspace}[2]{T_{#1} #2} % tangent space
\newcommand{\tangpt}{\ensuremath a}
\newcommand{\tangset}{\ensuremath A}
\newcommand{\taa}{\tspace{\tangpt}{\tangset}}
\newcommand{\tyy}{\tspace{\ipt}{\iset}}
%
% The set of admissible functions
\newcommand{\admiss}{\ensuremath \ms F}
\DeclareMathOperator{\arclen}{length}
%
% The objective functional
\newcommand{\objf}{\ensuremath \ms J}
\newcommand{\objp}{\ensuremath p}
\newcommand{\objfp}[1][\objp]{\objf_{#1}}
\newcommand{\objfpl}{\objf_\objp^\lambda}
\newcommand{\objell}{\ensuremath J}
\newcommand{\objellinfp}{\objell_\infty^+}
\newcommand{\wassp}{\wass_\objp}
\newcommand{\wpp}{\wass_\objp^\objp}
\newcommand{\wass}{\ensuremath \mbb W}
\newcommand{\otcost}{\ensuremath \mc T_c}
%
% First variation
\newcommand{\firstvar}{\ensuremath \delta \objfp\bk{\fmap; \pert}}
%
% The cost / constraint
\newcommand{\cost}{\ensuremath \ms C}
\newcommand{\costsf}{\ensuremath \msf C}
\newcommand{\budg}{\ensuremath \ell}
\newcommand{\budgmin}{\budg_{\rm min}}
\newcommand{\bnc}{\budg_{\rm nc}}
\newcommand{\hbudg}{\widehat \budg}
\newcommand{\bz}{\budg_0}
\newcommand{\bop}{\budg_1^+}
\newcommand{\bjp}{\budg_j^+}
\newcommand{\bjm}{\budg_j^-}
%
% Constraint ball
\newcommand{\cball}{\ms B}
\newcommand{\bell}{\cball_\budg}
\newcommand{\cflb}{\set{\cost(\fmap) \leq \budg}}
\newcommand{\cfl}[2][]{\ensuremath \set[#1]{\cost(\fmap) \leq {#2}}}
%
% Lebesgue measure
\newcommand{\leb}{\ensuremath \ms L}
\newcommand{\haus}{\ensuremath \mc H}
\newcommand{\hdim}{\ensuremath \dim_{\rm H}}
%%% Stuff for particular proofs
% Neural network macros
\newcommand{\nnnumlayers}{L}
\newcommand{\nnlayerindex}{l}
\newcommand{\nnffnet}{h}
\newcommand{\nnweight}{A}
\newcommand{\nnbias}{b}
\newcommand{\nnlatentdim}{d}
\newcommand{\nnposencoder}{\gamma}
\newcommand{\nnnonlin}{\sigma}
\newcommand{\nnbsize}{{\msf N}}
\newcommand{\nndataset}{D}
\newcommand{\nncand}{\msf{\dpt}}
\newcommand{\nnloss}{\mathcal{L}}
\newcommand{\nnlossobj}{\mathcal{L}_{\mathrm{obj}}}
\newcommand{\nnlosscost}{\mathcal{L}_{\mathrm{cost}}}
\newcommand{\nnlatent}{x}
\newcommand{\nnwdparam}{\lambda_{\mathrm{wd}}}
\newcommand{\learningrate}{\msf c}

%%% Formatting
%
% Cleverref configuration for special environments
\newlist{hyps}{enumerate}{1}
\setlist[hyps,1]{
    label={(H.\arabic*)},
    ref=(H.\arabic*), % if to be used with \cref, don't provide label string or parentheses
    wide,itemsep=0pt,topsep=0pt}
\creflabelformat{hypsi}{#2\textup{#1}#3} % note presence of parentheses
\crefname{hypsi}{Assumption}{Assumptions} % singular and plural forms of text labels
\Crefname{hypsi}{Assumption}{Assumptions}
% Cleverref for algorithms
\crefname{algocf}{Alg.}{Algs.}
\Crefname{algocf}{Algorithm}{Algorithms}



\newlist{hypsopt}{enumerate}{1}
\setlist[hypsopt,1]{
    label={(H*)},
    ref=(H*), % if to be used with \cref, don't provide label string or parentheses
    wide,itemsep=0pt,topsep=0pt}
\creflabelformat{hypsopti}{#2\textup{#1}#3} % note presence of parentheses
\crefname{hypsopti}{Assumption}{Assumptions} % singular and plural forms of text labels
\Crefname{hypsopti}{Assumption}{Assumptions}

% Custom referencing labels
\newcommand{\xref}{\nameref}
\makeatletter
\newcommand\xlabel[2][]{\phantomsection\def\@currentlabelname{#1}\label{#2}}
\makeatother

\newtcolorbox{defbox}{
  enhanced,
  sharp corners=all,
  colback=white,
  colframe=white,
  toprule=0pt,
  bottomrule=-1pt,
  leftrule=-6pt,
  rightrule=-6pt,
  overlay={
    \def\cornerlen{.75cm}
    \def\cornerwidth{.5pt}

    \fill[brown!10!white] (frame.north west) rectangle (frame.south east);

    \draw[line width=\cornerwidth] (frame.north west) -- ++(\cornerlen,0cm);
    \draw[line width=\cornerwidth] (frame.north west) -- ++(0cm,-\cornerlen);
    \draw[line width=\cornerwidth] (frame.south east) -- ++(-\cornerlen,0cm);
    \draw[line width=\cornerwidth] (frame.south east) -- ++(0cm,\cornerlen);
  }
}

% notation box
\newtcolorbox{notbox}[1][]{
  #1,
  breakable,
  enhanced,
  sharp corners=all,
  colback=white,
  colframe=white,
  grow to left by=-0em,%   equivalent to negative mdframed 'leftmargin'
  grow to right by=-0em,%   equivalent to negative mdframed 'leftmargin'
  toprule=0pt,
  bottomrule=-1pt,
  leftrule=-6pt,
  rightrule=-6pt,
  overlay={
    \def\cornerlen{.25cm}
    \def\cornerwidth{.5pt}

    % extra buffer
    \def\exbuff{0cm}

    \coordinate (nwe) at ($(frame.north west) + (\cornerlen, 0cm)$);
    \coordinate (nws) at ($(frame.north west) + (0, -\cornerlen)$);

    \coordinate (swe) at ($(frame.south west) + (\cornerlen, 0cm)$);
    \coordinate (swn) at ($(frame.south west) + (0, \cornerlen)$);

    \coordinate (new) at ($(frame.north east) + (-\cornerlen, 0cm)$);
    \coordinate (nes) at ($(frame.north east) + (0, -\cornerlen)$);

    \coordinate (sew) at ($(frame.south east) + (-\cornerlen, 0cm)$);
    \coordinate (sen) at ($(frame.south east) + (0, \cornerlen)$);

    \draw[line width=\cornerwidth/2, gray!50!white] (frame.north west)
    rectangle (frame.south east);

    \draw[line width=\cornerwidth]
    (nwe) --
    (frame.north west) --
    (nws);

    \draw[line width=\cornerwidth]
    (new) --
    (frame.north east) --
    (nes);

    \draw[line width=\cornerwidth]
    (swn) --
    (frame.south west) --
    (swe);

    \draw[line width=\cornerwidth]
    (sew) --
    (frame.south east) --
    (sen);
  }
}

\newenvironment{boxedremark}[1][]{\begin{notbox}\begin{remark}[#1] \small}{\end{remark}\end{notbox}}

